VectorNet: Encoding HD Maps and Agent Dynamics from Vectorized Representation

Behavior prediction in dynamic, multi-agent systems is an important problem in the context of self-driving cars, due to the complex representations and interactions of road components, including moving agents (e.g. pedestrians and vehicles) and road context information (e.g. lanes, traffic lights). This paper introduces VectorNet, a hierarchical graph neural network that first exploits the spatial locality of individual road components represented by vectors and then models the high-order interactions among all components. In contrast to most recent approaches, which render trajectories of moving agents and road context information as bird-eye images and encode them with convolutional neural networks (ConvNets), our approach operates on a vector representation. By operating on the vectorized high definition (HD) maps and agent trajectories, we avoid lossy rendering and computationally intensive ConvNet encoding steps. To further boost VectorNet's capability in learning context features, we propose a novel auxiliary task to recover the randomly masked out map entities and agent trajectories based on their context. We evaluate VectorNet on our in-house behavior prediction benchmark and the recently released Argoverse forecasting dataset. Our method achieves on par or better performance than the competitive rendering approach on both benchmarks while saving over 70% of the model parameters with an order of magnitude reduction in FLOPs. It also outperforms the state of the art on the Argoverse dataset.

==> sections/abstract_jiyang.tex <==
\begin{abstract}
   Behavior prediction is one of the core task in autonomous driving, where the goal is to predict the dynamics of other agents, like vehicles and pedestrians. Road maps play an important role in behavior prediction as they provide a strong prior for the task. Researchers have proposed many learning-based behavior prediction methods, most of them render the road map together with road agents on a sequence of images from top-down view, and use a convolutional neural network (CNN) to encode them. However rendering-based methods have many drawbacks, \eg it limits the input geometry range, long range road encoding and it's computationally expensive to render. To this end, we propose a vectorized representation for road geometry and agent dynamics, where the basic elements are polylines and vectors. We design a novel network architecture for such representation, called PolylineNet, which contains two major components: a Polyline Encoding Layer (PEL) to encode polyline features and a Polyline Interaction Graph (PIG) to reason the relations among road agents and road features. The evaluation is performed on the large scale Waymo Open Dataset, it outperforms the rendering-based methods while only needs 25\% of the parameters and 0.7\% of the computation cost compared with the CNN counterpart. \chen{we need to justify why using just maps and tracks.}
\end{abstract}

==> sections/experiments_jiyang.tex <==

\section{Experiments}
In this section, we present the datasets used, evaluation metrics and discuss the experimental results.

\subsection{Experimental Settings}

\subsubsection{Datasets} We use our in-house behavior prediction dataset and the Argoverse Forecasting for training and evaluation. We plan to release our dataset upon publication of the paper. Our in-house dataset is a unified multi-sensory dataset for perception and behavior prediction tasks. It contains lidar, camera, road map data and labels for 1000 segments. Each segment contains roughly 200 frames with length of 20s. Train and validation subsets have 798 and 202 segments respectively; the total number of trajectories sum up to 2.2M and 0.55M for train and validation set. There are abundant roadgraph features in the maps. We use lane boundaries, stop/yield signs, crosswalks and speed bumps in vectorized representations as model input.

Argoverse Forecasting~\cite{chang2019argoverse} is a trajectory-only dataset mined for behavior prediction task. It contains 211k sequences for training, 41k for validation, and 80k for testing, where each sequence contains one interesting vehicle trajectory for evaluation purposes. The core roadgraph features in the dataset are lane centerlines that vehicles should generally follow. Additional map features like traffic lights and stop signs are encoded as the attributes of the lanes.

\subsubsection{Metrics} For evaluation metrics, we adopt the widely used Average Displacement Error (ADE) and Displacement Error at T (DE@T) in meters.

\subsubsection{Rendering-based baselines} We render N consecutive past frames, each frame is a 400$\times$400$\times$3 image, which has road map component information and the perceived object bounding boxes. Rendering is based on the self-driving car's position in the most recent frame, and it is placed at the (200, 320), top-left corner is the image coordinate origin. N frames are stacked together to form a 400$\times$400$\times$3N image as model input.

Our baseline method is comparable to IntentNet: we use a ResNet-18 \cite{ResNet16} as the ConvNets backbone to process the rendered images. Unlike IntentNet, we do not use the lidar inputs. We crop the features along the history locations of the target track from the feature map, and average pool them to get a track feature. The track feature is fed into a fully connected layer (as used by IntentNet) to predict the future coordinates,  which is the same prediction head described in Section \ref{sec:head}. To test how ConvNets receptive field and feature cropping strategy influence the performance, we design several system variants: (1) Res18-k3+f1: crop a 1*1 feature patch at final location of the track (2) Res18-k3+f5: crop a 5*5 feature patch centered at the final location of the track, and avg-pool them; (3) Res18-k3+t1: crop a 1*1 feature patch at each history location of the track, and avg-pool them; (4) Res18-k5-t1: ResNet-18 with conv kernel size as 5, crop a 1*1 feature patch at each history location of the track, and avg-pool them; (5) Res18-k7: ResNet-18 with conv kernel size as 7, crop a 1*1 feature patch at each history location of the track, and avg-pool them.

The network is trained by an Adam optimizer \cite{kingma2014adam}, the learning rate is decayed every 5 epochs by a factor of 0.3. 

\subsubsection{VectorNet Implementation} We stack three PELs to encode polylines, all PELs use 64 unit for the fully connected layer.


\subsection{Evaluation on Waymo Open Dataset}
Comprehensive ablation study is done on Waymo Open Dataset for both rasterized representation and vectorized representation. For rasterized representation with ConvNets, we evaluate how rendering resolution and receptive field affect the performance and computational cost, and discuss the method limitations. For vectorized representation with VectorNet, we do various ablation studies to demonstrate its effectiveness and effciency.

\subsubsection{Rendering+ConvNets Evaluation.} 

\textbf{Representation Receptive Field.} As behavior prediction needs long range understanding of the road contexts, the representation receptive field is critical to the prediction quality. We evaluate different system variants to see how convolutional kernel size and feature cropping affect the prediction performance, as shown in Table \ref{tbl:rendered_od}. By comparing Res18-k3+t1, Res18-k5+t1 and Res18-k7+t1, it can be seen that enlarging the kernel size can slightly improve the performance, but the thing we need to keep in mind is that the computational cost also increases quadratically with the kernel size. For the feature cropping method, we can see that cropping larger feature patches (Res18-k3+f5 vs Res18-k3+f1) and history location features (Res18-k3+f1 vs Res18-k3+t1) can significantly improve the performance, and at the same time it doesn't introduce too much extra computation. The performance improvement also shows that the feature receptive field at each location of the ConvNets feature map is limited, it is necessary and critical to enlarge the feature context region for rendering+ConvNets based methods.

\begin{table}[!tb]
\centering
\begin{tabular}{c||c|c|c|c}\hline
Model       & DE@1      & DE@2  & DE@3          & ADE          \\\hline\hline
Res18-k3+f1  &  0.55   &  0.82  &  1.16      &     0.72      \\\hline
Res18-k3+f5   &   0.50   & 0.76  &   1.08      &     0.67     \\\hline
Res18-k3+t1  &     0.47   & 0.71 &     1.02     &    0.63  \\\hline
%Res18-Att  & k3+att & traj   &  0.50  &  1.08 & 0.66 \\\hline
Res18-k5+t1  &  0.46     & 0.71 &  1.00    &   0.62 \\\hline
Res18-k7+t1  &  0.45     & 0.70 &  1.00    &   0.61 \\\hline

\end{tabular}
\caption{Evaluation on representation receptive field for ConvNets on Open Dataset. DE and ADE are reported in meters.}\label{tbl:rendered_od}
\end{table}

\textbf{Rendering Resolution.} We vary rendering resolution to see how it affects the prediction quality and computational cost, as shown in Table \ref{tbl:resolution_od}. We use Res18-k3+t1 as the ConvNets backbone, and test three different resolutions, including 400*400 (0.25 meter per pixel), 200*200 (0.5 meter per pixel) and 100 * 100 (1 meter per pixel). 

\begin{table}[!tb]
\centering
\begin{tabular}{c||c|c|c|c}\hline
Resolution       & DE@1      & DE@2  & DE@3     & ADE          \\\hline\hline
100 * 100  &  0.57   &  0.84  &  1.17      &     0.74      \\\hline
200 * 200   &   0.51   & 0.77  &   1.10      &     0.67     \\\hline
400 * 400  &     0.47   & 0.71 &     1.02     &    0.63  \\\hline

\end{tabular}
\caption{Evaluation on representation receptive field for ConvNets on Open Dataset. DE and ADE are reported in meters.}\label{tbl:resolution_od}
\end{table}

\subsubsection{\model Evaluation.}

\begin{table}[!tb]
\centering
\begin{tabular}{c||c|c|c|c}\hline
Model       & DE@1      & DE@2  & DE@3          & ADE          \\\hline\hline
\model  &  0.53     & 0.74 &  1.00    &   0.67 \\\hline
\end{tabular}
\caption{Trajectory prediction performance on Open Dataset using vectorized representations. DE and ADE are reported in meters.}\label{tbl:vector_od}
\end{table}

\chen{There are a few sets of ablations we need to do. First, compare a flat graph with hierarchical graph. Second, compare different ways of modeling global interactions, such as vanilla attention, vanilla GCN and Transformers. Also compare with different depth, width and multiple heads. Third, verify that the auxiliary task actually helps.}


\subsubsection{Performance, FLOPs and Memory} 

In this section, we compare the performance, FLOPs and model size between ConvNets and VectorNet, which are shown in Table \ref{tbl:flops}. The prediction decoder is not counted for FLOPs and number of parameters. We can see that the FLOPs of ConvNets increasing quatratically with the kernel size and input image size; the number of parameters also increases quatratically with the kernel size.  When the performances are the same, it can be seen that ConvNets(Res18-k5+t1(400)) consumes 200+ times of FLOPs than VectorNet (15.81G vs 0.069G), and 7+ times of parameters (509K vs 72K). 

Note that the FLOPs is computed for a single predicting target. The FLOPs of VectorNet increases linearly with the number of predicting targets, as we need to re-normalize the vector coordinates for each target, and recompute the VectorNet feature. For the ConvNets, if the rendered images are target-centered, the FLOPs increases linearly with the number of targets; if the rendered images are self-driving-car-centered, then the feature map can be reused among multiple targets, the FLOPs is a constant number.

\begin{table}[!tb]
\centering
\begin{tabular}{c||c|c|c}\hline
Model       & FLOPs      & \#Param & DE@3 \\\hline\hline
Res18-k3+t1(100)  &     0.66G   & 246K  & 1.17\\\hline
Res18-k3+t1(200)  &     2.64G   & 246K &  1.10\\\hline
Res18-k3+t1(400)  &     10.56G  & 246K  &1.02 \\\hline
Res18-k5+t1(400)  &     15.81G   & 509K &1.00 \\\hline
Res18-k7+t1(400)  &     23.67G   & 902K &1.00 \\\hline \hline
VectorNet  &  0.069G     & 72K  & 1.00\\\hline

\end{tabular}
\caption{Model FLOPs and number of parameters comparison on ResNet and VectorNet. Prediction decoder is not counted for FLOPs and parameters.}\label{tbl:flops}
\end{table}


\subsection{Evaluation on Argoverse Forecasting Dataset}

We further conduct experiments on Argoverse Forecasting Dataset. Baselines include constant speed, weighted Nearest Neighbor, LSTM Encoder Decoder, and rendering-based model. We follow the rendering practice of Argoverse as 

\begin{table}[!tb]
\centering
\begin{tabular}{c||cccc}\hline
Model       & DE@1   & DE@3          & ADE          \\ \hline\hline
Constant Speed  &  -   &  -  &  -     \\\hline
Nearest Neighbor  &  -   &  -   &   -      \\\hline
LSTM ED  &  -   &  -   &   -      \\\hline
Res18-k3+f1  &  -   &  -  &  -      \\\hline
VectorNet  &  -   &  -  &  -       \\\hline
\end{tabular}
\caption{Trajectory prediction performance on Argoverse Forecasting Dataset. DE and ADE are reported in meters.}\label{tbl:rendered_argoverse}
\end{table}





==> sections/intro_jiyang.tex <==
\section{Introduction}

Behavior prediction is an important task in autonomous driving. Typically, it takes the perception outputs (\eg bounding box location, speed, acceleration, curvature) and predicts possible future trajectories based on road maps. A typical road map contains a set of well-defined road features, such as lanes, lane boundaries, crosswalks, speed-bumps and traffic lights; each road feature has a precise geographic extent. 

Traditional methods for behavior prediction are rule-based, road agents are assigned different types of behavior hypotheses based on the surrounding road features. Recently, researchers have proposed many learning-based behavior prediction methods \cite{casas2018intentnet, chai2019multipath, hong2019rules}. Most existing learning-based methods render the road map together with the dynamics of the road agents on an image from top-down view, and use a convolutional neural network (CNN) to encode road features and agent dynamics. The rendered images can align the road feature with other perception object bounding boxes well, and CNN can capture local interaction among objects and road features; however we observed it still suffers from the following issues:

1. Rendered images limit the input geometry range. The size of the rendered image and the required computation increase quadratically with the geometry range, thus it limits the geometry range we can use.

2. CNN receptive field limits the long-range geometry understanding.  CNN is effective to capture the local pattern by the convolution kernel. However, road features contains long-range geometry (lane boundaries, cross walks), which is significantly larger than normal convolutional receptive field.

3. Rendering is expensive. Typically, rendering a single 400 * 400 image on CPU needs 2 to 3 milliseconds; if we sequentially render 10 frames of history, then we need 20+ milliseconds, which can be a burden for onboard computation.

4. Rendering loses precision. Road features are represented in global coordinate system with precise location. Rendering needs to quantize the precise road coordinates to image pixel coordinate system, which loses precision.

To go beyond the limitations of the rendered images and CNN, we propose to encode the road map and road agents' dynamics directly from points, vectors and polylines. 
The geographic extent of the road features can be a point, a polygon, or a curve in geographic coordinates. For example, a lane boundary contains multiple control points that build a spline; a crosswalk is a polygon defined by several points; a stop sign is represented by a single point. All these geographic extent can be viewed as polylines defined by multiple control points; the road map within a certain region can be viewed as a set of polylines. Similarly, the road agents' trajectory can also be viewed as a polyline, where the control points are sampled from the original trajectory spline.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{cvpr-2020-vector.pdf}
    \caption{Vectorized representation for road features and road agents. \chen{Let's compare rendered and vectorized representations in this plot.}}
    \label{fig:vector}
\end{figure}

The key fact of those points and polylines are: The points in a polyline are ordered; the polylines in a scene (including the map polyline and agent trajectory polyline) are unordered. Given these facts, the next important formulation we make is converting points and polylines to vectors, where each vector is represented by [start point, end point, polyline type, polyline id]. Now ordered points in polylines become unordered vectors in polylines. In this way, we can represent the whole HD map by a set of such vectors.

Given such vectorized representation, we design a novel net architecture to encode the polylines from agent dynamics and road geometry, called PolylineNet. There are two sub-components: Polyline Encoding Layer (PEL) and Polyline Interaction Graph (PIG). A PEL takes the vectors as inputs and encodes the representations for each polyline; specifically, we first project the vectors to higher dimentional space (similar to PointNet \cite{qi2017pointnet}) by a multi-layer perceptron, and max-pool the vector features based on the polyline id of vectors, finally we gather the polyline feature back to each vector. A PIG builds the interaction graph among all polylines, so that each road agent is able to reason the relation with other road features and road agents, and gather the most useful information for future prediction.

In summary, our contributions are three-fold:

1. We propose a vectorized representation for road map and agent dynamics that can go beyong the limitations of rendered images. \chen{Are we the first to show on self-driving cars?}

2. We design a novel Polyline Encoding Layer (PEL) and Polyline Interaction Graph (PIG) to encode the vectorized representation.

3. We evaluate the proposed method on large scale Waymo Open Dataset, PolylineNet outperforms the rendered image + CNN method while only needs 10\% parameters of CNN counterpart.


==> sections/method_jiyang.tex <==
\section{Methods}
We first present how we represent agent dynamics and road features as polylines and vectors, then we talk about the basic building block Polyline Encoding Layer (PLE); finally we discuss how we build the relation graph over agent dynamics polylines and road feature polylines to gather interactive representations.

\subsection {Vectorized Representation}
For the road feature geometry, we sample points from the spline (\eg lanes, crosswalks) with a fixed spatial distance; for the agent dynamics (\ie past trajectory), we sample points with a fixed temporal interval. These sampled points are ordered, and they are used as the control points of the polylines, the polyline can either represent a road feature geometry or agent dynamics. A polyline vector is constructed by [start point, end point, polyline type, polyline id]. The polyline vectors are unordered, as we can rebuild the whole polyline without the ordering information of the vectors.

\subsection {Polyline Encoding Layer}
Given a set of vectors $\{vi\}$ and the associated polyline ids $\{p_i\}$, where $i$ is the vector index, a polyline layer projects the input vectors to another feature space. The vectors $\{v_i\}$ are first projected to a higher feature space by a encoder function $F(\cdot)$ (a single fully connected layer is used in our implementation), the outputs are vector features $\{f_i=F(v_i)\}$. To aggregate the information within a polyline, the vector features are max-pooled based on the polyline ids $\{p_i\}$ attached with each vector. Thus for a polyline $x$, the polyline feature $g_x = G(x) = \text{max-pool}(f_j)$, where $p_j=x$. A PEL can have two types of outputs, one is the per-vector features, the other is per-polyline features. To output the former one, the polyline feature $g_{p_i}$ is gathered back to each vector feature $f_i$, by concatenating them together $f'_i=\text{concat}(f_i, g_{p_i})$. The diagram for a single PEL is in Figure \ref{fig:pel}. There are two key designs in PEL:

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{cvpr-2020-pel.pdf}
    \caption{Vectorized representation for road features and road agents.}
    \label{fig:pel}
\end{figure}

\begin{itemize}
\item By converting the control points of a polyline to vectors, we convert the ordering among a set of points into vectors, so that the vectors are not ordered. 
\item We use the polyline id associated with each vector to gather the information for a polyline, and associate this information as a global context back to the vectors.
\end{itemize}
A single PLE can gather and aggregate the information from a set of vectors to a polyline. Multiple polyline layers stacked together allow the information propagate from vectors (local) to polylines (global).  


\subsection{Polyline Relation Reasoning}

To model the agent dynamics and road geometry, we use separate sets of stacked PELs to extract polyline features $g(p)$, shown in Figure \ref{fig:pil}. We note the agent dynamics polyline features as $g_a(p)$, and the road geometry polyline feature as $g_r(p)$, where $p$ represents an agent dynamic polyline or a road geometry polyline.
Given these polylines and their features, we build Polyline Interaction Graphs (PIG) on them. Generally, there are three types of graphs:

1. Agent-Road Graph: each agent can build relations with road polylines to distinguish most relevant nodes and less relevant nodes.

2. Agent Graph: to model dynamics among agents and how agents can influence each other.

3. Road Graph: to build a global roadgraph representation.

The edge between two nodes represents the relationship of them, every edge is associated with a score representing the relation intensity. The edge score is calculated by 
\begin{equation}
s(p, q) = \alpha(\phi_1(g(p)), \phi_2(g(q))) 
\end{equation}
where $\alpha$ is a distance function (cosine distance is used in our implementation) and $\phi$ is a mapping function (linear projection is used in our implementation). 

Given the relation edges among nodes, the per-agent feature $r(p)$ is gathered from road-agent graph and agent graph. Specifically, 
\begin{equation}
r_a(p) = \sum_q (s_a(p, q) g_a(q))
\end{equation}
\begin{equation}
r_{ar}(p) = \sum_q (s_{ar}(p, q) g_r(q))
\end{equation}
\begin{equation}
r(p) = \text{concat}(r_{ar}(p), r_{a}(p))
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{cvpr-2020-pig.pdf}
    \caption{Vectorized representation for road features and road agents.}
    \label{fig:pil}
\end{figure}
\subsection{Training Objectives}
\label{sec:head}
After gathering the relational information from graph for each agent, we use the produced feature to predict future trajectory by a multi-layer perceptron.

